OASIS: Optimal Arrangements for Sensing in SLAM

The number and arrangement of sensors on mobile robot dramatically influence its perception capabilities. Ensuring that sensors are mounted in a manner that enables accurate detection, localization, and mapping is essential for the success of downstream control tasks. However, when designing a new robotic platform, researchers and practitioners alike usually mimic standard configurations or maximize simple heuristics like field-of-view (FOV) coverage to decide where to place exteroceptive sensors. In this work, we conduct an information-theoretic investigation of this overlooked element of robotic perception in the context of simultaneous localization and mapping (SLAM). We show how to formalize the sensor arrangement problem as a form of subset selection under the E-optimality performance criterion. While this formulation is NP-hard in general, we show that a combination of greedy sensor selection and fast convex relaxation-based post-hoc verification enables the efficient recovery of certifiably optimal sensor designs in practice. Results from synthetic experiments reveal that sensors placed with OASIS outperform benchmarks in terms of mean squared error of visual SLAM estimates.

==> tables/compute_time.tex <==
% Please add the following required packages to your document preamble:

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\resizebox{0.98\linewidth}{!}{%
\begin{tabular}{llll}
\hline
\multicolumn{4}{c}{comparison of compute time} \\ \hline
Data      & Bruteforce    & greedy   & Convex Relaxation   \\ \hline
data 1    &               &          &         \\
data2     &               &          &         \\
data3     &               &          &         \\ \hline
\end{tabular}%
}
\caption{This table shows the comparison of the time taken by different approaches}
\label{tab:compute_algos}
\end{table}

==> tables/eval.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\captionsetup{font={footnotesize}, labelfont={bf,sf}}
\resizebox{\linewidth}{!}{%
\begin{tabular}{|l|ll|ll|ll|ll|ll|l|}
\hline
 &
  \multicolumn{2}{l|}{Greedy} &
  \multicolumn{2}{l|}{\begin{tabular}[c]{@{}l@{}}Cvx Relaxation\\ Rounded\end{tabular}} &
  \multicolumn{2}{l|}{Even} &
  \multicolumn{2}{l|}{Manual} &
  \multicolumn{2}{l|}{Random} &
  Cvx Relaxation \\ \hline
motion: circle & score  & rmse   & score  & rmse   & score  & rmse   & score  & rmse   & score  & rmse   & score  \\ \hline
k=2            & 0.256 & 0.395 & 0.073 & 0.639 & 0.072 & 0.343 & 0.069 & 1.164 & 0.022 & 0.670 & 0.386 \\
k=3            & 0.384 & 0.144 & 0.281 & 0.372 & 0.109 & 0.275 & 0.109 & 0.334 & 0.247 & 0.249 & 0.387 \\
k=4            & 0.386 & 0.076 & 0.359 & 0.215 & 0.159 & 0.206 & 0.386 & 0.150 & 0.384 & 0.134 & 0.387 \\
k=5            & 0.387 & 0.089 & 0.386 & 0.181 & 0.335 & 0.155 & 0.387 & 0.119 & 0.386 & 0.113 & 0.387 \\
k=6            & 0.388 & 0.070 & 0.387 & 0.153 & 0.387 & 0.135 & 0.387 & 0.112 & 0.387 & 0.087 & 0.388 \\ \hline
\end{tabular}%
}
\caption{This table shows the comparison of various benchmarking algorithms highlighting the advantages of set function maximization approaches discussed in this paper. \textcolor{red}{TODO: Fill out this table with new set of experiments}}
\label{tab:compute_algos}
\end{table}


% \begin{table}[]
% \captionsetup{font={footnotesize}, labelfont={bf,sf}}
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{|l|l|ll|ll|ll|ll|}
% \hline
%  &
%    &
%   \multicolumn{2}{l|}{RAND} &
%   \multicolumn{2}{l|}{EVEN} &
%   \multicolumn{2}{l|}{Greedy} &
%   \multicolumn{2}{l|}{Convex Relaxation} \\ \hline
%  &
%   Data &
%   Score &
%   rmse &
%   score &
%   rmse &
%   score &
%   rmse &
%   \multicolumn{1}{l|}{score} &
%   rmse \\ \hline
% \multirow{4}{*}{\begin{tabular}[c]{@{}l@{}}S\\ y\\ n\\ t\\ h\\ e\\ t\\ i\\ c\end{tabular}} &
%    &
%    &
%    &
%    &
%    &
%    &
%    &
%    &
%    \\
%  &  &  &  &  &  &  &  &  &  \\
%  &  &  &  &  &  &  &  &  &  \\
%  &  &  &  &  &  &  &  &  &  \\ \hline
% \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}R\\ e\\ a\\ l\end{tabular}} &
%    &
%    &
%    &
%    &
%    &
%    &
%    &
%    &
%    \\
%  &  &  &  &  &  &  &  &  &  \\ \hline
% \end{tabular}%
% }
% \caption{This table shows the comparison of various benchmarking algorithms highlighting the advantages of set function maximization approaches discussed in this paper. \textcolor{red}{TODO: Fill out this table with new set of experiments}}
% \label{tab:compute_algos}
% \end{table}
